Strategic Decision Support for AI Agents

Traditionally, decision support studies how humans use machine learning models to make better decisions. In modern agentic systems, this division of roles is increasingly reversed: AI agents act on behalf of users, while humans and tools becomes support mechanisms around them. This role reversal brings reliability concerns to the forefront, since agentic errors can be consequential and agent behavior must remain aligned with human goals and constraints. Departing from the classical view of decision support, we revisit its two basic principles, the cost--value tradeoff of seeking support and the role of uncertainty quantification, in a setting where AI agents are the central actors. We propose a framework for strategic decision support for AI agents through an optimization problem that minimizes support usage subject to controlling a counterfactual missed-support error: the probability that the agent acts alone on instances where support would have materially improved its output. At the population level, we show that the optimal policy is a threshold rule on the value of support. Building on this structure, we develop an online algorithm that adaptively thresholds such a score and uses randomized exploration to control missed-support error without distributional assumptions. We further introduce a calibration-on-the-fly method that reduces unnecessary support calls online. We instantiate this framework across diverse scenarios, including information gathering, human--AI collaboration, and tool use, showing how each can be modeled through the same strategic decision-support lens. Experiments across these settings show that our method reliably controls the target error while substantially reducing support usage in practice.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}
\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
\fi

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of our contributions and claims are properly explained in the abstract and introduction
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of our current work and possible avenues for future research in a separate section called Limitations and Future Work
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Due to space limit, we have moved all the proofs to the supplementary material, where we show full derivations of the proofs carefully, and clearly state all assumptions. We provide references for technical details as needed. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experimental setting is well explained in the main body of the paper, with specifics and all extra details of the implementations provided in the Appendix due to space limit. Further, we will publish our code for the camera ready version in case of acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will publish our code for the camera ready version in case of acceptance, and we will ensure instructions are clearly stated.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All details needed for a self-contained experiments section are provided in the main body, while further specifics and implementation details including all hyperparameters are provided in the Appendix for completeness and exact reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes we provide all necessary applicable statistics for a fair comparison.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To generate responses from the LLM, we can rely on API access which would remove the need for local GPU resources. The estimated total run-time of the experiments for this paper is in order of 3-5 hours, with majority of the time spent querying the LLM. The algorithm itself after these generations, runs in a matter of few minutes.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper has no forseeable ethical issues.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our framework is motivated by a societal concern which is ensuring that AI agents acting on behalf of users remain reliable and aligned with human intent as autonomy increases which will have positive societal impacts as discussed in Section~\ref{sec:intro}. We do not anticipate any negative societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not see any foreseeable need for safeguards.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have cited and credited all models and datasets used in our experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no new asset as an output.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: our experiments do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include such studies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core methods do not involve LLM as any important, original, or non-standard component. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> related_works.tex <==
https://arxiv.org/html/2409.00557v1

This one propmpts the LLM to ask when needed for clarifications from the user before calling the tool. 



\iffalse
%\cite{asai2023selfraglearningretrievegenerate} Our framework trains a single arbitrary LM that adaptively retrieves passages on-demand, and generates and reflects on retrieved passagesand its own generations using special tokens, called reflection tokens. Generating
reflection tokens makes the LM controllable during the inference phase, enabling it
to tailor its behavior to diverse task requirements. Experiments show that SELFRAG (7B and 13B parameters) significantly outperforms state-of-the-art LLMs
and retrieval-augmented models on a diverse set of tasks. 


\cite{Ijiang2023activeretrievalaugmentedgeneration} In
this work, we provide a generalized view of active retrieval augmented generation, methods
that actively decide when and what to retrieve
across the course of the generation. We propose
Forward-Looking Active REtrieval augmented
generation (FLARE), a generic method which
iteratively uses a prediction of the upcoming
sentence to anticipate future content, which is
then utilized as a query to retrieve relevant documents to regenerate the sentence if it contains
low-confidence tokens.


\cite{jeong2024adaptiveraglearningadaptretrievalaugmented} In this work, we
propose a novel adaptive QA framework that
can dynamically select the most suitable strategy for (retrieval-augmented) LLMs from the
simplest to the most sophisticated ones based
on the query complexity. Also, this selection process is operationalized with a classifier, which is a smaller LM trained to predict
the complexity level of incoming queries with
automatically collected labels, obtained from
actual predicted outcomes of models and inherent inductive biases in datasets. This approach offers a balanced strategy, seamlessly
adapting between the iterative and single-step
retrieval-augmented LLMs, as well as the noretrieval methods, in response to a range of
query complexities. 

\cite{han2024uncertaintyawarelanguageagent}, We present the Uncertainty-Aware Language Agent
(UALA), which improves a language agent’s efficiency in interaction with the external world to
answer various QA problems. We first measure the
uncertainty of an agent on a small set of examples
and establish an acceptable uncertainty threshold.
Then the uncertainty estimation function is integrated into a language agent’s trajectory of ThinkAct-Observe by measuring the uncertainty of generated answers, and then choosing to accept the
answer or to resort to external resources or human.
This approach does not require any training and the
language agent is prompted by few-shot learning.
We find that this technique significantly improves
the language agent’s performance on various QA
tasks (regardless of the backbone LLM size), and
offers a much more resource-efficient solution (substantially lower tool calling, and less number of
output tokens). We also show that UALA outperforms fine-tuning language agents in the presence
of small amount of data.



\cite{chen2023frugalgptuselargelanguage}  we propose FrugalGPT, a simple yet
flexible instantiation of LLM cascade which learns which combinations of LLMs to use for different
queries in order to reduce cost and improve accuracy. 

\cite{ong2025routellmlearningroutellms} Large language models (LLMs) excel at a wide range of tasks, but choosing the
right model often involves balancing performance and cost. Powerful models offer
better results but are expensive, while smaller models are more cost-effective but
less capable. To address this trade-off, we introduce a training framework for
learning efficient router models that dynamically select between a stronger and
weaker LLM during inference. Our framework leverages human preference data
and employs data augmentation techniques to enhance performance. Evaluations
on public benchmarks show that our approach can reduce costs by over 2 times
without sacrificing response quality. Moreover, our routers exhibit strong generalization capabilities, maintaining performance even when routing between LLMs
not included in training. This highlights the potential of our framework to deliver
cost-effective, high-performance LLM solutions.


\cite{zellinger2025costsavingllmcascadesearly} LLM cascades deploy small LLMs to answer most queries, limiting the use of large and expensive LLMs to difficult queries. This approach can significantly reduce costs without impacting performance. However, risk-sensitive domains such as finance or medicine place an additional premium on avoiding model errors. Since even the most expensive models are susceptible to making mistakes, applications in these domains benefit from allowing LLM systems to completely abstain from answering difficult queries. Introducing abstention poses a design question for LLM cascades: should abstention only be allowed at the final model or also at earlier models? Since the error patterns of small and large models are correlated, allowing earlier models to abstain may reduce inference costs and latency by anticipating abstention decisions by expensive and slow models, thus avoiding the need to run these models. We investigate the benefits of such "early abstention" in LLM cascades.

% Selective prediciton 
\cite{JMLR:v11:el-yaniv10a} We consider selective classification, a term we adopt here to refer to ‘classification with a reject option.’ The essence in selective classification is to trade-off classifier coverage for higher accuracy.
We term this trade-off the risk-coverage (RC) trade-off. Our main objective is to characterize this
trade-off and to construct algorithms that can optimally or near optimally achieve the best possible
trade-offs in a controlled manner. For noise-free models we present in this paper a thorough analysis of selective classification including characterizations of RC trade-offs in various interesting
settings. there is also \cite{geifman2017selectiveclassificationdeepneural, geifman2019selectivenetdeepneuralnetwork}.

%Learning to defer 
\cite{madras2018predictresponsiblyimprovingfairness} In many machine learning applications, there are multiple decision-makers involved, both automated and human. The interaction between these agents often goes unaddressed in algorithmic development. In this work, we explore a simple version of this interaction with a two-stage framework containing an automated model and an external decision-maker. The model can choose to say "Pass", and pass the decision downstream, as explored in rejection learning. We extend this concept by proposing "learning to defer", which generalizes rejection learning by considering the effect of other agents in the decision-making process. We propose a learning algorithm which accounts for potential biases held by external decision-makers in a system. Experiments demonstrate that learning to defer can make systems not only more accurate but also less biased. 

there is also \cite{mozannar2021consistentestimatorslearningdefer, verma2022calibratedlearningdeferonevsall}

Learning to defer extentions:\cite{verma2023learningdefermultipleexperts, NEURIPS2023_0b17d256} and \cite{montreuil2025optimalqueryallocationextractive}Large Language Models excel in generative tasks but exhibit inefficiencies in structured text selection, particularly in extractive question answering. This challenge is magnified in resource-constrained environments, where deploying multiple specialized models for different tasks is impractical. We propose a Learning-to-Defer framework that allocates queries to specialized experts, ensuring high-confidence predictions while optimizing computational efficiency. Our approach integrates a principled allocation strategy with theoretical guarantees on optimal deferral that balances performance and cost. Empirical evaluations on SQuADv1, SQuADv2, and TriviaQA demonstrate that our method enhances answer reliability while significantly reducing computational overhead, making it well-suited for scalable and efficient EQA deployment. 

Clarification seeking ( this could be more relevant to our work:) 

\cite{li2024inferencetimeinterventionelicitingtruthful} We introduce Inference-Time Intervention (ITI), a technique designed to enhance the "truthfulness" of large language models (LLMs). ITI operates by shifting model activations during inference, following a set of directions across a limited number of attention heads. This intervention significantly improves the performance of LLaMA models on the TruthfulQA benchmark.


(important to differentiate with this work) 
\cite{wang2026learningaskllmagents} Equipped with the capability to call functions, modern large language models (LLMs) can leverage external tools for addressing a range of tasks unattainable through language skills alone. However, the effective execution of these tools relies heavily not just on the advanced capabilities of LLMs but also on precise user instructions, which often cannot be ensured in the real world. To evaluate the performance of LLMs tool-use under imperfect instructions, we meticulously examine the real-world instructions queried from users, analyze the error patterns, and build a challenging tool-use benchmark called Noisy ToolBench (NoisyToolBench). We find that due to the next-token prediction training objective, LLMs tend to arbitrarily generate the missed argument, which may lead to hallucinations and risks. To address this issue, we propose a novel framework, Ask-when-Needed (AwN), which prompts LLMs to ask questions to users whenever they encounter obstacles due to unclear instructions. Moreover, to reduce the manual labor involved in user-LLM interaction and assess LLMs performance in tool utilization from both accuracy and efficiency perspectives, we design an automated evaluation tool named ToolEvaluator. Our experiments demonstrate that the AwN significantly outperforms existing frameworks for tool learning in the NoisyToolBench. We will release all related code and datasets to support future research. ( look at their related works too).


( for this work, and others along this theme and trainign theme, we can say were not focusing on triaing them to ask quesitons, which questiosn to ask. we dont do any training in general so even teianing to know when is not us that could be used as a stronger base). 
\cite{andukuri2024stargateteachinglanguagemodels}
When prompting language models to complete a task, users often leave important aspects unsaid. While asking questions could resolve this ambiguity (GATE; Li et al., 2023), models often struggle to ask good questions. We explore a language model's ability to self-improve (STaR; Zelikman et al., 2022) by rewarding the model for generating useful questions-a simple method we dub STaR-GATE. We generate a synthetic dataset of 25,500 unique persona-task prompts to simulate conversations between a pretrained language model-the Questioner-and a Roleplayer whose preferences are unknown to the Questioner. By asking questions, the Questioner elicits preferences from the Roleplayer. The Questioner is iteratively finetuned on questions that increase the probability of high-quality responses to the task, which are generated by an Oracle with access to the Roleplayer's latent preferences. After two iterations of self-improvement, the Questioner asks better questions, allowing it to generate responses that are preferred over responses from the initial model on


Uncertainty Gated thresholding:

\cite{kuhn2023clamselectiveclarificationambiguous}Users often ask dialogue systems ambiguous questions that require clarification. We show that current language models rarely ask users to clarify ambiguous questions and instead provide incorrect answers. To address this, we introduce CLAM: a framework for getting language models to selectively ask for clarification about ambiguous user questions. In particular, we show that we can prompt language models to detect whether a given question is ambiguous, generate an appropriate clarifying question to ask the user, and give a final answer after receiving clarification. We also show that we can simulate users by providing language models with privileged information. This lets us automatically evaluate multi-turn clarification dialogues. Finally, CLAM significantly improves language models' accuracy on mixed ambiguous and unambiguous questions relative to SotA.

Preference Optimizaiton and RL: 

\cite{zhang2025modelingfutureconversationturns} Large language models (LLMs) must often respond to highly ambiguous user requests. In such cases, the LLM's best response may be to ask a clarifying question to elicit more information. Existing LLMs often respond by presupposing a single interpretation of such ambiguous requests, frustrating users who intended a different interpretation. We speculate this is caused by current preference data labeling practice, where LLM responses are evaluated only on their prior contexts. To address this, we assign preference labels by simulating their expected outcomes in future turns. This allows LLMs to learn to ask clarifying questions when it can generate responses that are tailored to each user interpretation in future turns. On open-domain QA datasets with multiple annotations, we evaluate systems based on their ability to ask clarifying questions to recover each user's interpretation and expected answer. We compare systems trained using our proposed preference labeling methods against standard methods, which assign preferences based on only prior context.

\cite{Learning to Clarify: Multi-turn Conversations with Action-Based Contrastive Self-Training} Large language models (LLMs), optimized through human feedback, have rapidly emerged as a leading paradigm for developing intelligent conversational assistants. However, despite their strong performance across many benchmarks, LLM-based agents might still lack conversational skills such as disambiguation -- when they are faced with ambiguity, they often overhedge or implicitly guess users' true intents rather than asking clarification questions. Under task-specific settings, high-quality conversation samples are often limited, constituting a bottleneck for LLMs' ability to learn optimal dialogue action policies. We propose Action-Based Contrastive Self-Training (ACT), a quasi-online preference optimization algorithm based on Direct Preference Optimization (DPO), that enables data-efficient dialogue policy learning in multi-turn conversation modeling. We demonstrate ACT's efficacy under in data-efficient tuning scenarios, even when there is no action label available, using multiple real-world conversational tasks: tabular-grounded question-answering, machine reading comprehension, and AmbigSQL, a novel task for disambiguating information-seeking requests for complex SQL generation towards data analysis agents. Additionally, we propose evaluating LLMs' ability to function as conversational agents by examining whether they can implicitly recognize and reason about ambiguity in conversation. ACT demonstrates substantial conversation modeling improvements over standard tuning approaches like supervised fine-tuning and DPO.

\cite{qian2026scent} Augmenting large language models (LLMs) with external retrieval has become a standard method to address their inherent knowledge cutoff limitations. However, traditional retrieval-augmented generation methods employ static, pre-inference retrieval strategies, making them inadequate for complex tasks involving ambiguous, multi-step, or evolving information needs. Recent advances in test-time scaling techniques have demonstrated significant potential in enabling LLMs to dynamically interact with external tools, motivating the shift toward adaptive inference-time retrieval. Inspired by Information Foraging Theory (IFT), we propose InForage, a reinforcement learning framework that formalizes retrieval-augmented reasoning as a dynamic information-seeking process. Unlike existing approaches, InForage explicitly rewards intermediate retrieval quality, encouraging LLMs to iteratively gather and integrate information through adaptive search behaviors. To facilitate training, we construct a human-guided dataset capturing iterative search and reasoning trajectories for complex, real-world web tasks. Extensive evaluations across general question answering, multi-hop reasoning tasks, and a newly developed real-time web QA dataset demonstrate InForage's superior performance over baseline methods. These results highlight InForage's effectiveness in building robust, adaptive, and efficient reasoning agents. We provide all codes and datasets in the supplementary materials.

\cite{sun2025revisitingcommunicationefficiencymultiagent} Sun et al. (2025) formalized communication redundancy through a dimensional analysis of message embeddings and demonstrated that enforcing decorrelation within inter-agent representations significantly improves communication efficiency and cooperative performance in large-scale MARL systems.


%decision-theoretic objectives that weigh expected utility gain against an explicit asking cost

\cite{dong2026valueinformationframeworkhumanagent} Large Language Model (LLM) agents deployed for real-world tasks face a fundamental dilemma: user requests are underspecified, yet agents must decide whether to act on incomplete information or interrupt users for clarification. Existing approaches either rely on brittle confidence thresholds that require task-specific tuning, or fail to account for the varying stakes of different decisions. We introduce a decision-theoretic framework that resolves this trade-off through the Value of Information (VoI), enabling agents to dynamically weigh the expected utility gain from asking questions against the cognitive cost imposed on users. Our inference-time method requires no hyperparameter tuning and adapts seamlessly across contexts-from casual games to medical diagnosis. Experiments across four diverse domains (20 Questions, medical diagnosis, flight booking, and e-commerce) show that VoI consistently matches or exceeds the best manually-tuned baselines, achieving up to 1.36 utility points higher in high-cost settings. This work provides a parameter-free framework for adaptive agent communication that explicitly balances task risk, query ambiguity, and user effort.

\cite{overman2025conformalarbitrageriskcontrolledbalancing} Modern language model deployments must often balance competing objectives, for example, helpfulness versus harmlessness, cost versus accuracy, and reward versus safety. We introduce Conformal Arbitrage, a post hoc framework that learns a data driven threshold to mediate between a Primary model optimized for a primary objective and a more conservative Guardian which could be another model or a human domain expert aligned with a guardrail objective. The threshold is calibrated with conformal risk control, yielding finite sample, distribution free guarantees that the long run frequency of undesirable events, such as factual errors or safety violations, does not exceed a user specified quota. Because Conformal Arbitrage operates wholly at the API level, without requiring access to model logits or updating model weights, it complements weight based alignment techniques and integrates seamlessly with existing cost aware cascades. Empirically, Conformal Arbitrage traces an efficient frontier, allowing users to define an acceptable performance level for one objective while maximizing utility in another. We observe that our method outperforms, in terms of accuracy, cost matched random routing between models. These properties make Conformal Arbitrage a practical, theoretically grounded tool for trustworthy and economical deployment of large language models across a broad range of potentially competing objectives.


\cite{okati2021differentiablelearningtriage} Multiple lines of evidence suggest that predictive models may benefit from algorithmic triage. Under algorithmic triage, a predictive model does not predict all instances but instead defers some of them to human experts. However, the interplay between the prediction accuracy of the model and the human experts under algorithmic triage is not well understood. In this work, we start by formally characterizing under which circumstances a predictive model may benefit from algorithmic triage. In doing so, we also demonstrate that models trained for full automation may be suboptimal under triage. Then, given any model and desired level of triage, we show that the optimal triage policy is a deterministic threshold rule in which triage decisions are derived deterministically by thresholding the difference between the model and human errors on a per-instance level. Building upon these results, we introduce a practical gradient-based algorithm that is guaranteed to find a sequence of triage policies and predictive models of increasing performance. Experiments on a wide variety of supervised learning tasks using synthetic and real data from two important applications -- content moderation and scientific discovery -- illustrate our theoretical results and show that the models and triage policies provided by our gradient-based algorithm outperform those provided by several competitive baselines.

\cite{ross2025when2callnottools}Leveraging external tools is a key feature for modern Language Models (LMs) to expand their capabilities and integrate them into existing systems. However, existing benchmarks primarily focus on the accuracy of tool calling -- whether the correct tool is called with the correct parameters -- and less on evaluating when LMs should (not) call tools. We develop a new benchmark, When2Call, which evaluates tool-calling decision-making: when to generate a tool call, when to ask follow-up questions and when to admit the question can't be answered with the tools provided. We find that state-of-the-art tool-calling LMs show significant room for improvement on When2Call, indicating the importance of this benchmark. We also develop a training set for When2Call and leverage the multiple-choice nature of the benchmark to develop a preference optimization training regime, which shows considerably more improvement than traditional fine-tuning. We release the benchmark and training data as well as evaluation scripts at this

\cite{pona2026calibratethendelegatesafetymonitoringrisk} Monitoring LLM safety at scale requires balancing cost and accuracy: a cheap latent-space probe can screen every input, but hard cases should be escalated to a more expensive expert. Existing cascades delegate based on probe uncertainty, but uncertainty is a poor proxy for delegation benefit, as it ignores whether the expert would actually correct the error. To address this problem, we introduce Calibrate-Then-Delegate (CTD), a model-cascade approach that provides probabilistic guarantees on the computation cost while enabling instance-level (streaming) decisions. CTD builds on a novel delegation value (DV) probe, a lightweight model operating on the same internal representations as the safety probe that directly predicts the benefit of escalation. To enforce budget constraints, CTD calibrates a threshold on the DV signal using held-out data via multiple hypothesis testing, yielding finite-sample guarantees on the delegation rate. Evaluated on four safety datasets, CTD consistently outperforms uncertainty-based delegation at every budget level, avoids harmful over-delegation, and adapts budget allocation to input difficulty without requiring group labels.

\cite{ren2023robotsaskhelpuncertainty}Large language models (LLMs) exhibit a wide range of promising capabilities -- from step-by-step planning to commonsense reasoning -- that may provide utility for robots, but remain prone to confidently hallucinated predictions. In this work, we present KnowNo, which is a framework for measuring and aligning the uncertainty of LLM-based planners such that they know when they don't know and ask for help when needed. KnowNo builds on the theory of conformal prediction to provide statistical guarantees on task completion while minimizing human help in complex multi-step planning settings. Experiments across a variety of simulated and real robot setups that involve tasks with different modes of ambiguity (e.g., from spatial to numeric uncertainties, from human preferences to Winograd schemas) show that KnowNo performs favorably over modern baselines (which may involve ensembles or extensive prompt tuning) in terms of improving efficiency and autonomy, while providing formal assurances. KnowNo can be used with LLMs out of the box without model-finetuning, and suggests a promising lightweight approach to modeling uncertainty that can complement and scale with the growing capabilities of foundation models. 
% these papers I could not find \citep{frank2012predicting,goodman2016pragmatic,hawkins2015why,sumers2021how, so need to know what their titles are. 


\cite{kapoor2025largelanguagemodelstaught}When using large language models (LLMs) in high-stakes applications, we need to know when we can trust their predictions. Some works argue that prompting high-performance LLMs is sufficient to produce calibrated uncertainties, while others introduce sampling methods that can be prohibitively expensive. In this work, we first argue that prompting on its own is insufficient to achieve good calibration and then show that fine-tuning on a small dataset of correct and incorrect answers can create an uncertainty estimate with good generalization and small computational overhead. We show that a thousand graded examples are sufficient to outperform baseline methods and that training through the features of a model is necessary for good performance and tractable for large open-source models when using LoRA. We also investigate the mechanisms that enable reliable LLM uncertainty estimation, finding that many models can be used as general-purpose uncertainty estimators, applicable not just to their own uncertainties but also the uncertainty of other models. Lastly, we show that uncertainty estimates inform human use of LLMs in human-AI collaborative settings through a user study.

\cite{liu2024uncertaintyestimationquantificationllms}
In this paper, we study the problem of uncertainty estimation and calibration for LLMs. We begin by formulating the uncertainty estimation problem, a relevant yet underexplored area in existing literature. We then propose a supervised approach that leverages labeled datasets to estimate the uncertainty in LLMs' responses. Based on the formulation, we illustrate the difference between the uncertainty estimation for LLMs and that for standard ML models and explain why the hidden neurons of the LLMs may contain uncertainty information. Our designed approach demonstrates the benefits of utilizing hidden activations to enhance uncertainty estimation across various tasks and shows robust transferability in out-of-distribution settings. We distinguish the uncertainty estimation task from the uncertainty calibration task and show that better uncertainty estimation leads to better calibration performance. Furthermore, our method is easy to implement and adaptable to different levels of model accessibility including black box, grey box, and white box.

\cite{li2025conftunertraininglargelanguage}Large Language Models (LLMs) are increasingly deployed in high-stakes domains such as science, law, and healthcare, where accurate expressions of uncertainty are essential for reliability and trust. However, current LLMs are often observed to generate incorrect answers with high confidence, a phenomenon known as "overconfidence". Recent efforts have focused on calibrating LLMs' verbalized confidence: i.e., their expressions of confidence in text form, such as "I am 80\% confident that...". Existing approaches either rely on prompt engineering or fine-tuning with heuristically generated uncertainty estimates, both of which have limited effectiveness and generalizability. Motivated by the notion of proper scoring rules for calibration in classical machine learning models, we introduce ConfTuner, a simple and efficient fine-tuning method that introduces minimal overhead and does not require ground-truth confidence scores or proxy confidence estimates. ConfTuner relies on a new loss function, tokenized Brier score, which we theoretically prove to be a proper scoring rule, intuitively meaning that it "correctly incentivizes the model to report its true probability of being correct". ConfTuner improves calibration across diverse reasoning tasks and generalizes to black-box models such as GPT-4o. Our results further show that better-calibrated confidence enables downstream gains in self-correction and model cascade, advancing the development of trustworthy LLM systems. The code is available at this https URL.
The baove htree is really just methods that try to express uncertainty better. anything that does training a probe could be done on top of our method to get a better confidence signal that the support will help or not. But i think just worth mentioning something along the lines that the LLM's uncertainty about the output is differnt question than whether the support would help ornot.



\subsection{Methodological Neighbors}
\label{app:related-methods}

Our online algorithm and finite-sample guarantee draw on three
methodological lines, none of which directly addresses support-seeking
but each of which contributes to the techniques we use.

\paragraph{Conformal prediction and risk control.}
Conformal prediction~\citep{vovk2005algorithmic,angelopoulos2021gentle}
provides distribution-free coverage guarantees by calibrating thresholds
on a held-out set. Risk-controlling prediction
sets~\citep{bates2021distribution} extend the framework from coverage to
general bounded losses. Applications to LLMs include conformal
factuality~\citep{mohri2024conformal} and conformal
abstention~\citep{yadkori2024mitigating}.

\paragraph{Online risk control under distribution shift.}
\citet{gibbs2021adaptive} introduced adaptive conformal inference, which
updates the conformal threshold online to maintain coverage under
distribution shift. Subsequent work refined the threshold update for
faster convergence and stronger
guarantees~\citep{angelopoulos2024online,gibbs2024conformal,bastani2022practical}.
Our threshold update belongs to this lineage but differs in two ways:
(i) the target is a conditional rather than marginal error, and (ii)
the feedback is partial, revealed only on rounds where support is
sought, which motivates the importance-weighted update and the
randomized exploration in Algorithm~\ref{alg:ads}.

\paragraph{Neyman--Pearson classification.}
Neyman--Pearson classification~\citep{scott2005neyman,tong2013plugin}
minimizes one error type subject to an upper bound on another, and is
the classical statistical formulation matching our optimization
problem~\eqref{SDS-Opt}. Existing online NP
classifiers~\citep{can2020online} update Lagrangian thresholds with full
label feedback. Our setting differs in that the constraint involves a
counterfactual benefit indicator observable only on rounds where
support is invoked, requiring the partial-feedback machinery developed
in Section~\ref{sec:algo}.



\section{Extended Related Works}
\section{Extended Related Works}
\label{app:related}

This section expands the discussion of Section~\ref{sec:related}. We organize
prior work along the same three axes used in the main body --- training
agents to seek support, allocating tasks across decision-making systems, and
inference-time policies for support-seeking --- and add two further
subsections covering the uncertainty estimation literature that produces
candidate score signals, and the methodological lines that underpin our
finite-sample guarantee.

\subsection{Training Agents to Seek Support}
\label{app:related-training}

A large body of work bakes support-seeking behavior into the agent itself
through training. We expand on two threads of this line. Both serve as
stronger \emph{base agents} on top of which our oversight layer operates,
rather than as competing approaches: the agent is trained to be more capable
at the underlying support modality, and our framework wraps the resulting
agent.

\paragraph{Tool use and adaptive retrieval.}
Toolformer~\citep{schick2023toolformerlanguagemodelsteach} is a
self-supervised method that teaches a language model where to insert API
calls during generation by sampling and filtering candidate calls based on
whether they reduce future-token loss. Self-RAG~\citep{asai2023selfraglearningretrievegenerate}
trains a model to interleave retrieval with generation through special
reflection tokens that signal when to retrieve, when to critique retrieved
passages, and when to commit to an answer. Confidence-triggered retrieval
methods take a complementary route, deciding to retrieve based on signals
during decoding: FLARE~\citep{Ijiang2023activeretrievalaugmentedgeneration}
uses next-sentence prediction to anticipate content and triggers retrieval
when the predicted sentence contains low-confidence tokens; Adaptive-RAG~\citep{jeong2024adaptiveraglearningadaptretrievalaugmented}
trains a small classifier that predicts query complexity and routes among
no-retrieval, single-step, and iterative-retrieval strategies; UALA~\citep{han2024uncertaintyawarelanguageagent}
sets an uncertainty threshold on agent answers and resorts to external
resources when the threshold is exceeded; and SCENT~\citep{qian2026scent}
formalizes adaptive retrieval as a reinforcement learning problem with
dense rewards on intermediate retrieval quality.

\paragraph{Training agents to ask.}
A second thread trains the agent to ask the user for clarification rather
than to invoke an external tool. Generative Active Task Elicitation
(GATE)~\citep{li2023eliciting} introduced the framework of having an LLM
elicit user preferences through targeted questions, providing the
foundation for subsequent training-based approaches. STaR-GATE~\citep{andukuri2024stargateteachinglanguagemodels}
fine-tunes a Questioner model on synthetic dialogues to maximize the
probability of high-quality downstream responses. ACT introduces an
action-based contrastive self-training procedure --- a DPO-style preference
optimization at the conversational-action level --- to teach LLMs to
disambiguate before answering. Other work labels preference data by
simulating expected outcomes of future
turns~\citep{zhang2025modelingfutureconversationturns}, or trains models on
benchmarks that explicitly evaluate the ask-or-tool-call decision~\citep{ross2025when2callnottools}.
AwN~\citep{wang2026learningaskllmagents} prompts LLMs to ask questions when
they encounter unclear instructions during tool use; while not strictly a
training method, it likewise modifies the agent's generation strategy to
incorporate asking.

\paragraph{Relation to our framework.}
All of the above produce stronger base agents: a model that has been
trained to call SQL appropriately, to retrieve when needed, or to ask
informative clarifying questions is precisely the kind of policy our
oversight layer sits on top of. Our experiments use state-of-the-art LLMs
(Qwen-2.5-7B, Gemini-2.5-Flash, GPT-4o-mini) that already incorporate
substantial training of this kind, and our gains are reported on top of
these strong agents. Our framework does not modify the agent's weights or
generation procedure, so any of these training methods can be deployed
together with our algorithm.

\subsection{Allocating Tasks Across Decision-Making Systems}
\label{app:related-routing}

A second body of work studies how to allocate tasks across multiple
decision-making systems, rather than how to support a single one. We
distinguish four sub-directions, each of which solves a structurally
different problem from ours.

\paragraph{Cascades and routers.}
LLM cascades and routers send each query to the cheapest system whose
output is good enough.
FrugalGPT~\citep{chen2023frugalgptuselargelanguage} composes LLM APIs into
a cascade with learned stop criteria, using progressively stronger models
only when needed. RouteLLM~\citep{ong2025routellmlearningroutellms} trains
a router that selects between strong and weak LLMs using human preference
data. Cost-saving cascades with early
abstention~\citep{zellinger2025costsavingllmcascadesearly} extend cascades
to allow abstention at intermediate tiers, leveraging the correlation
between small- and large-model errors. The decision in all of these is
\emph{which system answers the query}.

\paragraph{Learning to defer.}
Learning to defer routes uncertain instances to an expert whose decision
\emph{replaces} the model's. The framework was introduced by~\citet{madras2018predictresponsiblyimprovingfairness}
as a generalization of rejection learning that accounts for downstream
decision-makers. Subsequent work developed Bayes-consistent surrogate
losses~\citep{mozannar2021consistentestimatorslearningdefer}, calibrated
one-vs-all approaches~\citep{verma2022calibratedlearningdeferonevsall},
extensions to multiple
experts~\citep{verma2023learningdefermultipleexperts,NEURIPS2023_0b17d256},
and applications to LLM
allocation~\citep{montreuil2025optimalqueryallocationextractive}.
\citet{okati2021differentiablelearningtriage} characterizes the optimal
deferral policy as a per-instance threshold on the difference between
model and expert errors, and provides a gradient-based algorithm to learn
it. The decision in all of these is whose answer is used.

\paragraph{Selective prediction and abstention.}
Selective prediction lets the model abstain entirely on uncertain inputs,
trading coverage for accuracy~\citep{JMLR:v11:el-yaniv10a,geifman2017selectiveclassificationdeepneural,geifman2019selectivenetdeepneuralnetwork}.
The decision is whether anyone answers at all.

\paragraph{Conformal-calibrated routing.}
A more recent line uses conformal calibration to deliver formal guarantees
on routing or delegation decisions. Conformal
Arbitrage~\citep{overman2025conformalarbitrageriskcontrolledbalancing}
calibrates a threshold to mediate between a primary model and a more
conservative guardian model, providing finite-sample distribution-free
guarantees on the rate of undesirable events.
Calibrate-Then-Delegate~\citep{pona2026calibratethendelegatesafetymonitoringrisk}
introduces a delegation-value probe that predicts the benefit of
escalating to an expert, and calibrates a threshold on this probe via
offline multiple-hypothesis testing. CTD is the closest of the cited works
to our algorithm at the methodological level: it shares the idea of a
probe predicting benefit-of-help, and a calibrated threshold over this
probe. The substantive differences are that (i) CTD operates in a routing
setting where the expert's decision replaces the model's, whereas our
agent retains output ownership; (ii) CTD requires offline calibration on
a held-out set, whereas our threshold is updated fully online without one;
and (iii) CTD controls a marginal delegation rate, whereas we control a
conditional counterfactual error.

\paragraph{Relation to our framework.}
The unifying feature across this entire line is that the decision is
about \emph{who produces the output}, or whether it is produced at all.
In our setting the same agent always produces the output, and support is
auxiliary information --- a clarifying question, a tool result,
additional evidence, or expert guidance --- that the agent itself
incorporates into its reasoning. Routing and abstention machinery does
not directly apply because there is no second decision-maker to route to,
and no abstention option in our framework.

\subsection{Inference-Time Policies for Support-Seeking}
\label{app:related-asking}

This is the line most closely related to our work. We give a fuller
treatment of the three families summarized in Section~\ref{sec:related},
emphasizing the policy machinery of each method and what each requires of
its support modality. We also note the broader thread of decision-theoretic
frameworks for LLM agents, which addresses an adjacent but distinct
question.

\paragraph{Heuristic confidence thresholding.}
The simplest approach triggers help-seeking when a confidence signal about
the agent's own answer falls below a hand-tuned threshold.
CLAM~\citep{kuhn2023clamselectiveclarificationambiguous} prompts an LLM
to classify whether a question is ambiguous, and asks a clarifying
question when it is. AwN~\citep{wang2026learningaskllmagents} prompts the
LLM to ask whenever it encounters obstacles caused by unclear instructions
during tool use. When2Call~\citep{ross2025when2callnottools} evaluates
models on the ask-or-act decision and trains them via preference
optimization on multiple-choice action labels. Earlier proactive-dialogue
work uses prompting to elicit clarifying behavior more
generally~\citep{deng2023prompting}. The signal in all of these is the
LLM's confidence in its own answer, and the threshold is fixed
heuristically or through training. No formal control over the rate at
which support is missed when it would have helped is provided.

\paragraph{Decision-theoretic asking.}
A more principled approach computes the expected utility of asking under
an explicit asking cost. The recent Value-of-Information policy
of~\citet{dong2026valueinformationframeworkhumanagent} maintains a belief
distribution $b(\theta)$ over latent user intents, generates a small set
of candidate clarifying questions via an LLM, simulates plausible user
replies for each candidate question (using the LLM as a surrogate for
the user), updates the belief to a hypothetical posterior under each
simulated reply, and computes the value of asking as the expected utility
of the post-asking decision minus the value of acting now. The agent
asks when the maximum value-of-information across candidate questions
exceeds a fixed asking-cost coefficient. This policy is parameter-free
in the sense that there is no threshold to tune, but it requires (i) a
discrete set of candidate user intents to enumerate, (ii) an LLM-based
simulator for user replies, (iii) a known utility function $U(\theta, a)$
over agent actions and latent intents, and (iv) a calibrated belief
distribution over intents. Each of these is naturally available when
support is a clarifying question about user intent --- the modality the
method is designed for --- but is not naturally available for the support
modalities in our experiments: there are no candidate questions to
enumerate when support is SQL execution against a table, no simulator
over user replies when support is additional clinical evidence, and no
utility function over latent intents when support is a stronger
reasoner's guidance on a specific math step.

\paragraph{Conformal-set asking.}
KnowNo~\citep{ren2023robotsaskhelpuncertainty} uses split conformal
prediction on a held-out calibration set to construct a prediction set
over candidate intents at coverage level $1-\alpha$, and asks for help
whenever the resulting set is non-singleton. The guarantee is on
\emph{marginal coverage} --- the prediction set contains the true intent
with probability at least $1-\alpha$ over the input distribution --- and
the calibration is offline and one-shot. KnowNo applies cleanly when the
support-relevant uncertainty can be expressed as a discrete prediction
set over options, which is natural for the user-intent setting it was
designed for. It does not directly apply to support modalities whose
support-relevant uncertainty is not expressible as a label set.

\paragraph{Decision theory for LLM agents more broadly.}
A separate thread applies decision-theoretic frameworks to LLM agents at
the level of action selection rather than information acquisition,
typically by reasoning about expected utility under fixed information
about the task or
user~\citep{liu2024decisiontheoreticllm,lin2024decision,chen2025decisiontheoretic}.
Our framework shares the decision-theoretic spirit of this line but
addresses the upstream question of when the agent should seek further
information before acting --- a question that is logically prior to the
action-selection problem these works study.

\paragraph{Relation to our framework.}
The three asking families above each address a specific instantiation of
support-seeking: confidence thresholding, decision-theoretic asking, and
conformal-set asking are all designed around the case where support is
a clarifying question about user intent, and their policy machinery
reflects this. Our framework brings these approaches under common design
principles: a score that targets the counterfactual benefit of seeking
support, and a threshold rule that controls a conditional missed-support
error online. This gives three properties absent from each of the above:
(i) the algorithm applies uniformly across support modalities --- tools,
evidence, expert guidance, and clarifying questions --- without modality-
specific machinery; (ii) it operates fully online, without an offline
calibration set or task-specific hyperparameter tuning; and (iii) it
provides finite-sample distribution-free control over the conditional
rate at which support is missed when it would have helped, at a
user-specified level $\alpha$.

\subsection{Uncertainty Estimation in LLMs}
\label{app:related-uncertainty}

Our framework requires a score $s_\theta(x) \in [0,1]$ that quantifies
how likely it is that seeking support would change the agent's output.
The quality of this score determines how often support is invoked at a
given target error level, but \emph{not} whether the error is controlled,
which is guaranteed by Theorem~\ref{thm:mse}. A separate literature
studies how to elicit reliable uncertainty estimates from LLMs.~\citet{kapoor2025largelanguagemodelstaught}
shows that fine-tuning on a small set of correct/incorrect answers
produces well-calibrated confidence with small computational overhead,
and that internal-feature training is necessary for
reliability.~\citet{liu2024uncertaintyestimationquantificationllms}
proposes a supervised uncertainty estimator based on hidden activations,
demonstrating transferability to out-of-distribution
settings.~\citet{li2025conftunertraininglargelanguage} introduces
ConfTuner, which fine-tunes for verbalized confidence using a tokenized
Brier-score loss with proper-scoring-rule guarantees.

We emphasize a conceptual distinction that is important for our setting:
the agent's confidence in its answer and the benefit of seeking support
are different quantities. An agent can be confidently wrong in cases
where support would flip its output, and confidently right in cases
where support is redundant; the two quantities diverge precisely on the
consequential cases. The anchored score family in
Section~\ref{sec:scores} uses self-reported confidence as a starting
signal but learns a residual correction toward the benefit-of-support
target via calibration-on-the-fly. Better LLM uncertainty estimators
from this line could be used as the anchor in our anchored score,
providing a stronger initial signal that calibration-on-the-fly need
only refine; we view this complementarity as straightforward and leave
its empirical study to future work.

